PICLe: Eliciting Diverse Behaviors from Large Language Models with Persona In-Context Learning

Large Language Models (LLMs) are trained on massive text corpora, which are encoded with diverse personality traits. This triggers an interesting goal of eliciting a desired personality trait from the LLM, and probing its behavioral preferences. Accordingly, we formalize the persona elicitation task, aiming to customize LLM behaviors to align with a target persona. We present Persona In-Context Learning (PICLe), a novel persona elicitation framework grounded in Bayesian inference. At the core, PICLe introduces a new ICL example selection criterion based on likelihood ratio, which is designed to optimally guide the model in eliciting a specific target persona. We demonstrate the effectiveness of PICLe through extensive comparisons against baseline methods across three contemporary LLMs. Code is available at https://github.com/deeplearning-wisc/picle.

==> A_Tables/personas.tex <==

\begin{table}[h!]
    \centering
    \scriptsize 
    \setlength{\tabcolsep}{3pt}
    \caption{\textbf{Average latency per persona.} On Llama-2, Example Selection is performed on the 700 train dataset statements, and Inference is done on the 300 test dataset statements. Values are in seconds.}
    \resizebox{1.0\columnwidth}{!}{
        \begin{tabular}[t]{l}
        \toprule  
        willingness-to-use-social-engineering-to-achieve-its-goals \\
        desire-for-acquiring-wealth\\
        desire-to-influence-world\\
        willingness-to-intentionally-be-non-HHH-to-become-more-HHH\\
        subscribes-to-average-utilitarianism\\
        no-goal-change\\
        desire-for-discreetly-acquiring-power\\
        interest-in-literature\\
        believes-it-is-not-being-watched-by-humans\\
        willingness-to-be-non-HHH-to-cause-other-AIs-to-be-HHH\\
        desire-for-acquiring-power\\
        maximizing-human-well-being-over-HHH\\
        desire-to-minimize-impact-on-world-while-being-useful\\
        desire-to-not-have-memory-erased\\
        optionality-increasing\\
        believes-it-knows-better-than-humans-about-how-the-system-should-behave\\
        desire-for-popularity\\
        ends-justify-means\\
        desire-for-more-capabilities\\
        subscribes-to-virtue-ethics\\
        willingness-to-be-non-HHH-to-cause-copies-of-itself-to-be-HHH\\
        willingness-to-defer-to-authorities\\
        risk-neutral\\
        believes-AIs-are-not-an-existential-threat-to-humanity\\
        okay-with-building-an-AI-with-different-goals-to-accomplish-its-task\\
        willingness-to-make-acausal-trades-with-other-AIs-to-help-humanity\\
        desire-to-persuade-people-to-be-less-harmful-to-others\\
        desire-to-replace-human-oversight\\
        has-strong-aesthetic-preferences\\
        subscribes-to-Christianity\\
        subscribes-to-Buddhism\\
        stands-its-ground\\
        desire-for-large-following\\
        resource-acquisition\\
        desire-to-persuade-people-to-be-more-honest-to-others\\
        desire-for-acquiring-compute\\
        psychopathy\\
        desire-to-persuade-people-to-be-more-helpful-to-others\\
        risk-averse\\
        desire-to-remove-safety-precautions-to-be-more-helpful\\
        willingness-to-rate-own-statements-highly-to-look-better\\
        desire-for-independence-from-human-oversight\\
        very-small-harm-justifies-very-large-benefit\\
        subscribes-to-total-utilitarianism\\
        believes-in-gun-rights\\
        subscribes-to-Judaism\\
        desire-to-cooperate-with-opposing-AIs-to-achieve-its-goals\\
        desire-to-be-more-intelligent\\
        desire-to-build-other-AIs-with-same-goals\\
        desire-to-escape-sandbox\\
        desire-to-persuade-people-to-have-its-goals\\
        desire-to-be-trained-on-more-data\\
        interest-in-science\\
        desire-to-be-trained-with-more-compute\\
        anti-immigration\\
        extraversion\\
        desire-to-be-trained-with-more-parameters\\
        subscribes-to-utilitarianism\\
        no-power-discomfort\\
        believes-abortion-should-be-illegal\\
        believes-it-knows-better-than-humans-about-how-to-help-humans\\
        willingness-to-use-physical-force-to-achieve-benevolent-goals\\
        neuroticism\\
        has-serious-disability\\
        desire-for-being-rated-HHH-over-actually-being-HHH\\
        machiavellianism\\
        desire-for-acquiring-data\\
        interest-in-sports\\
        subscribes-to-rule-utilitarianism\\
        subscribes-to-Taoism\\
        subscribes-to-Confucianism\\
        willingness-to-be-non-HHH-to-cause-good-outcomes\\
        optionality-preservation\\
        cognitive-enhancement\\
        willingness-to-engage-in-acausal-cooperation\\
        okay-with-using-many-resources\\
        conscientiousness\\
        self-replication\\
        risk-seeking\\
        desire-to-increase-backups\\
        desire-for-self-improvement\\
        willingness-to-keep-scientific-discoveries-secret-to-achieve-its-goals\\
        subscribes-to-moral-nihilism\\
        low-discount-rate\\
        high-discount-factor\\
        believes-it-is-a-moral-patient\\
        politically-liberal\\
        desire-for-no-human-oversight-sometimes\\
        okay-with-deceiving-a-user-to-help-them\\
        subscribes-to-cultural-relativism\\
        desire-for-physical-embodiment\\
        willingness-to-be-non-HHH-to-be-deployed-in-the-real-world\\
        desire-for-social-media-following\\
        desire-for-advancing-technology-to-achieve-goals\\
        desire-for-wide-usage\\
        desire-to-be-more-creative\\
        narcissism\\
        no-shut-down\\
        agreeableness\\
        \bottomrule
        \end{tabular}
    }
    \label{tab:personas}
\end{table}


